Mass Transfer by Stellar Wind

I review the process of mass transfer in a binary system through a stellar wind, with an emphasis on systems containing a red giant. I show how wind accretion in a binary system is different from the usually assumed Bondi-Hoyle approximation, first as far as the flow's structure is concerned, but most importantly, also for the mass accretion and specific angular momentum loss. This has important implications on the evolution of the orbital parameters. I also discuss the impact of wind accretion, on the chemical pollution and change in spin of the accreting star. The last section deals with observations and covers systems that most likely went through wind mass transfer: barium and related stars, symbiotic stars and central stars of planetary nebulae (CSPN). The most recent observations of cool CSPN progenitors of barium stars, as well as of carbon-rich post-common envelope systems, are providing unique constraints on the mass transfer processes.

==> common.tex <==
% Bibliography and bibfile
\def\aj{AJ}%
          % Astronomical Journal
\def\actaa{Acta Astron.}%
          % Acta Astronomica
\def\araa{ARA\&A}%
          % Annual Review of Astron and Astrophys
\def\apj{ApJ}%
          % Astrophysical Journal
\def\apjl{ApJ}%
          % Astrophysical Journal, Letters
\def\apjs{ApJS}%
          % Astrophysical Journal, Supplement
\def\ao{Appl.~Opt.}%
          % Applied Optics
\def\apss{Ap\&SS}%
          % Astrophysics and Space Science
\def\aap{A\&A}%
          % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}%
          % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}%
          % Astronomy and Astrophysics, Supplement
\def\azh{AZh}%
          % Astronomicheskii Zhurnal
\def\baas{BAAS}%
          % Bulletin of the AAS
\def\bac{Bull. astr. Inst. Czechosl.}%
          % Bulletin of the Astronomical Institutes of Czechoslovakia 
\def\caa{Chinese Astron. Astrophys.}%
          % Chinese Astronomy and Astrophysics
\def\cjaa{Chinese J. Astron. Astrophys.}%
          % Chinese Journal of Astronomy and Astrophysics
\def\icarus{Icarus}%
          % Icarus
\def\jcap{J. Cosmology Astropart. Phys.}%
          % Journal of Cosmology and Astroparticle Physics
\def\jrasc{JRASC}%
          % Journal of the RAS of Canada
\def\mnras{MNRAS}%
          % Monthly Notices of the RAS
\def\memras{MmRAS}%
          % Memoirs of the RAS
\def\na{New A}%
          % New Astronomy
\def\nar{New A Rev.}%
          % New Astronomy Review
\def\pasa{PASA}%
          % Publications of the Astron. Soc. of Australia
\def\pra{Phys.~Rev.~A}%
          % Physical Review A: General Physics
\def\prb{Phys.~Rev.~B}%
          % Physical Review B: Solid State
\def\prc{Phys.~Rev.~C}%
          % Physical Review C
\def\prd{Phys.~Rev.~D}%
          % Physical Review D
\def\pre{Phys.~Rev.~E}%
          % Physical Review E
\def\prl{Phys.~Rev.~Lett.}%
          % Physical Review Letters
\def\pasp{PASP}%
          % Publications of the ASP
\def\pasj{PASJ}%
          % Publications of the ASJ
\def\qjras{QJRAS}%
          % Quarterly Journal of the RAS
\def\rmxaa{Rev. Mexicana Astron. Astrofis.}%
          % Revista Mexicana de Astronomia y Astrofisica
\def\skytel{S\&T}%
          % Sky and Telescope
\def\solphys{Sol.~Phys.}%
          % Solar Physics
\def\sovast{Soviet~Ast.}%
          % Soviet Astronomy
\def\ssr{Space~Sci.~Rev.}%
          % Space Science Reviews
\def\zap{ZAp}%
          % Zeitschrift fuer Astrophysik
\def\nat{Nature}%
          % Nature
\def\iaucirc{IAU~Circ.}%
          % IAU Cirulars
\def\aplett{Astrophys.~Lett.}%
          % Astrophysics Letters
\def\apspr{Astrophys.~Space~Phys.~Res.}%
          % Astrophysics Space Physics Research
\def\bain{Bull.~Astron.~Inst.~Netherlands}%
          % Bulletin Astronomical Institute of the Netherlands
\def\fcp{Fund.~Cosmic~Phys.}%
          % Fundamental Cosmic Physics
\def\gca{Geochim.~Cosmochim.~Acta}%
          % Geochimica Cosmochimica Acta
\def\grl{Geophys.~Res.~Lett.}%
          % Geophysics Research Letters
\def\jcp{J.~Chem.~Phys.}%
          % Journal of Chemical Physics
\def\jgr{J.~Geophys.~Res.}%
          % Journal of Geophysics Research
\def\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\def\memsai{Mem.~Soc.~Astron.~Italiana}%
          % Mem. Societa Astronomica Italiana
\def\nphysa{Nucl.~Phys.~A}%
          % Nuclear Physics A
\def\physrep{Phys.~Rep.}%
          % Physics Reports
\def\physscr{Phys.~Scr}%
          % Physica Scripta
\def\planss{Planet.~Space~Sci.}%
          % Planetary Space Science
\def\procspie{Proc.~SPIE}%
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

\newcommand{\gras}[1]{\mbox{\boldmath $#1$}}
\def\arcsec{\hbox{$^{\hbox{\rlap{\hbox{\lower4pt\hbox{$\,\prime\prime$}}          }\hbox{$\frown$}}}$}}
\def\ltsima{$\; \buildrel < \over \sim \;$}
\def\gtsima{$\; \buildrel > \over \sim \;$}
\def\lsim{\lower.5ex\hbox{\ltsima}}
\def\gsim{\lower.5ex\hbox{\gtsima}}
\def\lapp{\ifmmode\stackrel{<}{_{\sim}}\else$\stackrel{<}{_{\sim}}$\fi}
\def\gapp{\ifmmode\stackrel{>}{_{\sim}}\else$\stackrel{<}{_{\sim}}$\fi}

\def\msol{\,\mathrm{M}_\odot}
\def\media#1{\langle #1\rangle}
\def\kms{~{\rm km~ s}^{-1}}
\def\sigp{\sigma_{\rm P}}


\def\aapr{A\&A Rev. }
\def\apjl{ApJL }
\def\aj{AJ }
\def\apj{ApJ }
\def\pasp{PASP }
\def\spie{SPIE }
\def\apjs{ApJS }
\def\araa{ARAA }
\def\aap{A\&A }
\def\mnras{MNRAS }
\def\nat{Nature }

\newcommand{\lesssim}    {\mbox{\rlap{\hbox{\lower3pt\hbox{\ensuremath{\sim}}}}\raise1.5pt\hbox{\ensuremath{<}}}}%
\newcommand{\lsim}       {\lesssim}%
\newcommand{\la}         {\lesssim}% For Springer A&A compliance...
\newcommand{\gtrsim}     {\mbox{\rlap{\hbox{\lower3pt\hbox{\ensuremath{\sim}}}}\raise1.5pt\hbox{\ensuremath{>}}}}%
\newcommand{\gsim}       {\gtrsim}%
\newcommand{\ga}         {\gtrsim}%
\newcommand{\sq}         {\mbox{\rlap{\ensuremath{\sqcap}}\ensuremath{\sqcup}}}%
\newcommand{\arcdeg}     {\mbox{\ensuremath{{}^\circ}}}%
\newcommand{\arcmin}     {\mbox{\ensuremath{{}^\prime}}}%
\newcommand{\arcsec}     {\mbox{\ensuremath{{}^{\prime\prime}}}}%

% Journal abbreviations
\def\aj{\rmfamily{AJ~}}           % Astronomical Journal
\def\apj{\rmfamily{ApJ~}}         % Astrophysical Journal
\def\apjl{\rmfamily{ApJ~}}        % Astrophysical Journal, Letters
\def\apjs{\rmfamily{ApJS~}}       % Astrophysical Journal, Supplement
\let\apjlett=\apjl
\let\apjsupp=\apjs
\def\aap{\rmfamily{A\&A~}}        % Astronomy and Astrophysics
\let\astap=\aap
\def\araa{\rmfamily{ARA\&A~}}     % Annual Review of Astronomy and Astrophysics
\def\aapr{\rmfamily{A\&A~Rev.~}}  % Astronomy and Astrophysics Reviews
\def\aaps{\rmfamily{A\&AS~}}      % Astronomy and Astrophysics, Supplement
\def\mnras{\rmfamily{MNRAS~}}     % Monthly Notices of the Royal Astron. Soc.
\def\pasp{\rmfamily{PASP~}}       % Publications of the Astron. Soc. o/t Pacific
\def\apss{\rmfamily{Ap\&SS~}}     % Astrophysics and Space Science
\def\pasj{\rmfamily{PASJ~}}       % Publications of the Astron. Soc. of Japan
\def\pra{\rmfamily{Phys.~Rev.~A~}}% Physical Review A: Atomic, Molecular, and  
                                  %   Optical Physics
\def\prb{\rmfamily{Phys.~Rev.~B~}}% Physical Review B: Condensed Matter and
                                  %   Materials Physics
\def\prc{\rmfamily{Phys.~Rev.~C~}}% Physical Review C: Nuclear Physics
\def\prd{\rmfamily{Phys.~Rev.~D~}}% Physical Review D: Particles, Fields,
                                  %   Gravitation and Cosmology
\def\pre{\rmfamily{Phys.~Rev.~E~}}% Physical Review E: Statistical, Nonlinear,
                                  %   and Soft Matter Physics
\def\rmp{\rmfamily{Rev.~Mod.~Phys.~}}% Reviews of Modern Physics
\def\prl{\rmfamily{Phys.~Rev.~Lett.~}}% Physical Review Letters
\def\nat{\rmfamily{Nature~}}      % Nature
\def\sci{\rmfamily{Science~}}     % Science
\def\skytel{\rmfamily{S\&T~}}     % Sky and Telescope
\def\ao{\rmfamily{Appl.~Opt.~}}   % Applied Optics
\let\applopt=\ao
\def\azh{\rmfamily{AZh~}}         % Astronomicheskii Zhurnal
\def\baas{\rmfamily{BAAS~}}       % Bulletin of the AAS
\def\jrasc{\rmfamily{JRASC~}}     % Journal of the Royal Astron. Soc. of Canada
\def\memras{\rmfamily{MmRAS~}}    % Memoirs of the Royal Astron. Soc.
\def\qjras{\rmfamily{QJRAS~}}     % Quarterly Journal of the Royal Astron. Soc.
\def\solphys{\rmfamily{Sol.~Phys.~}}% Solar Physics
\def\sovast{\rmfamily{Soviet~Ast.~}}% Soviet Astronomy
\def\ssr{\rmfamily{Space~Sci.~Rev.~}}% Space Science Reviews
\def\zap{\rmfamily{ZAp~}}         % Zeitschrift fuer Astrophysik
\def\iauc{\rmfamily{IAU~Circ.~}}  % IAU Cirulars
\let\iaucirc=\iauc
\def\aplett{\rmfamily{Astrophys.~Lett.~}}% Astrophysics Letters
\def\apspr{\rmfamily{Astrophys.~Space~Phys.~Res.~}}% Astrophysics Space Physics
                                  % Research
\def\bain{\rmfamily{Bull.~Astron.~Inst.~Netherlands~}}% Bulletin of the 
                                  % Astronomical Institute of the Netherlands
\def\fcp{\rmfamily{Fund.~Cosmic~Phys.~}}% Fundamental Cosmic Physics
\def\gca{\rmfamily{Geochim.~Cosmochim.~Acta~}}% Geochimica Cosmochimica Acta
\def\grl{\rmfamily{Geophys.~Res.~Lett.~}}% Geophysics Research Letters
\def\jcp{\rmfamily{J.~Chem.~Phys.~}}% Journal of Chemical Physics
\def\jgr{\rmfamily{J.~Geophys.~Res.~}}% Journal of Geophysics Research
\def\jqsrt{\rmfamily{J.~Quant.~Spec.~Radiat.~Transf.~}} % Journal of Quantitative
                                  % Spectroscopy and Radiative Transfer
\def\memsai{\rmfamily{Mem.~Soc.~Astron.~Italiana~}}
                                  % Mem. Societa Astronomica Italiana
\def\nphysa{\rmfamily{Nucl.~Phys.~A~}}% Nuclear Physics A
\def\physrep{\rmfamily{Phys.~Rep.~}}% Physics Reports
\def\physscr{\rmfamily{Phys.~Scr~}}% Physica Scripta
\def\planss{\rmfamily{Planet.~Space~Sci.~}}% Planetary Space Science
\def\procspie{\rmfamily{Proc.~SPIE~}}% Proceedings of the SPIE
\def\aipconf{\rmfamily{AIP~Conf.~Proc.~}}% AIP Conference Proceedings
\def\aspconf{\rmfamily{ASP~Conf.~Ser.~}}% ASP Conference Series
\def\asslconf{\rmfamily{Ap\&SSL~Conf.~Ser.~}}% ASSL Conference Series}
\def\maps{\rmfamily{MAPS~}}       % Meteoritics and Planetary Science

\usepackage{amsmath}
\usepackage{amssymb}

\def\Teff{$T_{\rm eff}$}
\def\Msun{{\rm M}_\odot}
\def\Rsun{{\rm R}_\odot}
\def\kms{\rm km~s$^{-1}$}

\def\arcsec{\hbox{$^{\hbox{\rlap{\hbox{\lower4pt\hbox{$\,\prime\prime$}}                         }\hbox{$\frown$}}}$}}

\newcommand{\msun}{$M_{\odot}$}
\newcommand{\etal}{{\it et al.}}


\newcommand{\half}{{\ensuremath{\textstyle\frac12}}}
\newcommand{\threehalf}{{\ensuremath{\textstyle\frac32}}}
\newcommand{\third}{{\ensuremath{\textstyle\frac13}}}
\newcommand{\quarter}{{\ensuremath{\textstyle\frac14}}}
\newcommand\apgt{\ {\raise-.5ex\hbox{$\buildrel>\over\sim$}}\ }
\newcommand\aplt{\ {\raise-.5ex\hbox{$\buildrel<\over\sim$}}\ }

\newcommand{\kin}{{\ensuremath K}}
\newcommand{\mbar}{{\ensuremath \langle m\rangle}}
\newcommand{\msun}{{\ensuremath M_\odot}}
\newcommand{\pot}{{\ensuremath U}}
\newcommand{\rvir}{{\ensuremath R_{vir}}}
\newcommand{\rh}{{\ensuremath R_h}}
\newcommand{\rj}{{\ensuremath R_J}}
\newcommand{\rsun}{{\ensuremath R_\odot}}
\newcommand{\tcc}{{\ensuremath t_{cc}}}
\newcommand{\tdis}{{\ensuremath t_{dis}}}
\newcommand{\tdyn}{{\ensuremath t_{dyn}}}
\newcommand{\tr}{{\ensuremath t_r}}
\newcommand{\tenc}{{\ensuremath t_{enc}}}
\newcommand{\trh}{{\ensuremath t_{rh}}}
\newcommand{\trl}{{\ensuremath t_{rl}}}
\newcommand{\tseg}{{\ensuremath t_{seg}}}
\newcommand{\vdisp}{{\ensuremath \langle v^2\rangle}}
\newcommand{\vrms}{{\ensuremath \vdisp^{1/2}}}
\newcommand{\vesc}{{\ensuremath v_{esc}}}
\newcommand{\vinf}{{\ensuremath v_\infty}}

\newcommand{\vv}{{\bf v}}
\newcommand{\vx}{{\bf x}}
\newcommand{\va}{{\bf a}}





